Quantifying Disorder One Atom at a Time Using an Interpretable Graph Neural Network Paradigm

Quantifying the level of atomic disorder within materials is critical to understanding how evolving local structural environments dictate performance and durability. Here, we leverage graph neural networks to define a physically interpretable metric for local disorder. This metric encodes the diversity of the local atomic configurations as a continuous spectrum between the solid and liquid phases, quantified against a distribution of thermal perturbations. We apply this novel methodology to three prototypical examples with varying levels of disorder: (1) solid-liquid interfaces, (2) polycrystalline microstructures, and (3) grain boundaries. Using elemental aluminum as a case study, we show how our paradigm can track the spatio-temporal evolution of interfaces, incorporating a mathematically defined description of the spatial boundary between order and disorder. We further show how to extract physics-preserved gradients from our continuous disorder fields, which may be used to understand and predict materials performance and failure. Overall, our framework provides an intuitive and generalizable pathway to quantify the relationship between complex local atomic structure and coarse-grained materials phenomena.

==> bib.tex <==
@article{fey2019fast,
  title={Fast graph representation learning with PyTorch Geometric},
  author={Fey, Matthias and Lenssen, Jan Eric},
  journal={arXiv preprint arXiv:1903.02428},
  year={2019}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@inproceedings{smith2019super,
  title={Super-convergence: Very fast training of neural networks using large learning rates},
  author={Smith, Leslie N and Topin, Nicholay},
  booktitle={Artificial Intelligence and Machine Learning for Multi-Domain Operations Applications},
  volume={11006},
  pages={1100612},
  year={2019},
  organization={International Society for Optics and Photonics}
}

@article{paszke2019pytorch,
  title={Pytorch: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={8026--8037},
  year={2019}
}

@article{bresson2017residual,
  title={Residual gated graph convnets},
  author={Bresson, Xavier and Laurent, Thomas},
  journal={arXiv preprint arXiv:1711.07553},
  year={2017}
}

@article{dwivedi2020benchmarking,
  title={Benchmarking graph neural networks},
  author={Dwivedi, Vijay Prakash and Joshi, Chaitanya K and Laurent, Thomas and Bengio, Yoshua and Bresson, Xavier},
  journal={arXiv preprint arXiv:2003.00982},
  year={2020}
}

@Article{Fish2021,
author={Fish, Jacob
and Wagner, Gregory J.
and Keten, Sinan},
title={Mesoscopic and multiscale modelling in materials},
journal={Nature Materials},
year={2021},
month={Jun},
day={01},
volume={20},
number={6},
pages={774-786},
}

@article{Miller_2009,
	doi = {10.1088/0965-0393/17/5/053001},
	url = {https://doi.org/10.1088/0965-0393/17/5/053001},
	year = 2009,
	month = {may},
	publisher = {{IOP} Publishing},
	volume = {17},
	number = {5},
	pages = {053001},
	author = {Ronald E Miller and E B Tadmor},
	title = {A unified framework and performance benchmark of fourteen multiscale atomistic/continuum coupling methods},
	journal = {Modelling and Simulation in Materials Science and Engineering},
}

@article{KARMA201625,
title = {Atomistic to continuum modeling of solidification microstructures},
journal = {Current Opinion in Solid State and Materials Science},
volume = {20},
number = {1},
pages = {25-36},
year = {2016},
note = {Recent Advances in Solidification Microstructure- Experiments and Computational Analysis},
issn = {1359-0286},
doi = {https://doi.org/10.1016/j.cossms.2015.09.001},
url = {https://www.sciencedirect.com/science/article/pii/S1359028615300061},
author = {Alain Karma and Damien Tourret},
}

@article{doi:10.1063/1.2423084,
author = {Srinivasan,S. G.  and Baskes,M. I.  and Wagner,G. J. },
title = {Atomistic simulations of shock induced microstructural evolution and spallation in single crystal nickel},
journal = {Journal of Applied Physics},
volume = {101},
number = {4},
pages = {043504},
year = {2007},
doi = {10.1063/1.2423084},

URL = { 
        https://doi.org/10.1063/1.2423084
    
},
eprint = { 
        https://doi.org/10.1063/1.2423084
    
}

}

@article{LIU2021110733,
title = {Atomistic simulation of microstructure evolution of NiTi single crystals in bending deformation},
journal = {Computational Materials Science},
volume = {199},
pages = {110733},
year = {2021},
issn = {0927-0256},
doi = {https://doi.org/10.1016/j.commatsci.2021.110733},
url = {https://www.sciencedirect.com/science/article/pii/S0927025621004602},
author = {Shan Liu and Yao Lin and Luyi Han and Xiebin Wang and Guoqun Zhao and Guangchun Wang},
}

@article{SIMON2010106,
title = {Detection and analysis of hot-spot formation in solar cells},
journal = {Solar Energy Materials and Solar Cells},
volume = {94},
number = {2},
pages = {106-113},
year = {2010},
issn = {0927-0248},
doi = {https://doi.org/10.1016/j.solmat.2009.09.016},
url = {https://www.sciencedirect.com/science/article/pii/S0927024809003420},
author = {Michael Simon and Edson L. Meyer},
}

@article{doi:10.1021/j100111a031,
author = {Tokmakoff, A. and Fayer, M. D. and Dlott, Dana D.},
title = {Chemical reaction initiation and hot-spot formation in shocked energetic molecular materials},
journal = {The Journal of Physical Chemistry},
volume = {97},
number = {9},
pages = {1901-1913},
year = {1993},
doi = {10.1021/j100111a031},

URL = { 
        https://doi.org/10.1021/j100111a031
    
},
eprint = { 
        https://doi.org/10.1021/j100111a031
    
}

}

@article{BUDEVSKI20002559,
title = {Electrocrystallization: Nucleation and growth phenomena},
journal = {Electrochimica Acta},
volume = {45},
number = {15},
pages = {2559-2574},
year = {2000},
issn = {0013-4686},
doi = {https://doi.org/10.1016/S0013-4686(00)00353-4},
url = {https://www.sciencedirect.com/science/article/pii/S0013468600003534},
author = {E. Budevski and G. Staikov and W.J. Lorenz},
}

@article{doi:10.1021/cr2001756,
author = {Zhang, Renyi and Khalizov, Alexei and Wang, Lin and Hu, Min and Xu, Wen},
title = {Nucleation and Growth of Nanoparticles in the Atmosphere},
journal = {Chemical Reviews},
volume = {112},
number = {3},
pages = {1957-2011},
year = {2012},
doi = {10.1021/cr2001756},
    note ={PMID: 22044487},

URL = { 
        https://doi.org/10.1021/cr2001756
    
},
eprint = { 
        https://doi.org/10.1021/cr2001756
    
}

}

@article{Curtin_2003,
	doi = {10.1088/0965-0393/11/3/201},
	url = {https://doi.org/10.1088/0965-0393/11/3/201},
	year = 2003,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {11},
	number = {3},
	pages = {R33--R68},
	author = {W A Curtin and Ronald E Miller},
	title = {Atomistic/continuum coupling in computational materials science},
	journal = {Modelling and Simulation in Materials Science and Engineering},
}

@article{doi:10.1063/1.4959168,
author = {Wagner,Jacob W.  and Dama,James F.  and Durumeric,Aleksander E. P.  and Voth,Gregory A. },
title = {On the representability problem and the physical meaning of coarse-grained models},
journal = {The Journal of Chemical Physics},
volume = {145},
number = {4},
pages = {044108},
year = {2016},
doi = {10.1063/1.4959168},

URL = { 
        https://doi.org/10.1063/1.4959168
    
},
eprint = { 
        https://doi.org/10.1063/1.4959168
    
}

}

@article{Stukowski_2012,
	doi = {10.1088/0965-0393/20/4/045021},
	year = 2012,
	publisher = {{IOP} Publishing},
	volume = {20},
	number = {4},
	pages = {045021},
	author = {Alexander Stukowski},
	title = {Structure identification methods for atomistic simulations of crystalline materials},
	journal = {Model Simul. Mat. Sci. Eng.}
}

@article{doi:10.1080/01418618108235816,
author = { Paul J.   Steinhardt  and  P.   Chaudhari },
title = {Point and line defects in glasses},
journal = {Philos. Mag. A},
volume = {44},
number = {6},
pages = {1375-1381},
year  = {1981},
publisher = {Taylor & Francis},
doi = {10.1080/01418618108235816},


}

@article{PhysRevB.73.054104,
  title = {Applications of local crystal structure measures in experiment and simulation},
  author = {Ackland, G. J. and Jones, A. P.},
  journal = {Phys. Rev. B},
  volume = {73},
  pages = {054104},
  numpages = {7},
  year = {2006},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.73.054104},
}

﻿@Article{Rosenbrock2017,
author={Rosenbrock, Conrad W.
and Homer, Eric R.
and Cs{\'a}nyi, G{\'a}bor
and Hart, Gus L. W.},
title={Discovering the building blocks of atomic systems using machine learning: application to grain boundaries},
journal={npj Computational Materials},
year={2017},
month={Aug},
day={03},
volume={3},
number={1},
pages={29},
}

@article{doi:10.1073/pnas.1807176115,
author = {Tristan A. Sharp  and Spencer L. Thomas  and Ekin D. Cubuk  and Samuel S. Schoenholz  and David J. Srolovitz  and Andrea J. Liu },
title = {Machine learning determination of atomic dynamics at grain boundaries},
journal = {Proceedings of the National Academy of Sciences},
volume = {115},
number = {43},
pages = {10943-10947},
year = {2018},
doi = {10.1073/pnas.1807176115},
}

@Article{C6CP00415F,
author ="De, Sandip and Bartók, Albert P. and Csányi, Gábor and Ceriotti, Michele",
title  ="Comparing molecules and solids across structural and alchemical space",
journal  ="Phys. Chem. Chem. Phys.",
year  ="2016",
volume  ="18",
pages  ="13754-13769",
publisher  ="The Royal Society of Chemistry",
doi  ="10.1039/C6CP00415F",
}

@article{doi:10.1063/1.3553717,
author = {Behler,Jörg },
title = {Atom-centered symmetry functions for constructing high-dimensional neural network potentials},
journal = {J. Chem. Phys.},
volume = {134},
number = {7},
pages = {074106},
year = {2011},
doi = {10.1063/1.3553717},
}


@article{doi:10.1137/15M1054183,
author = {Shapeev, Alexander V.},
title = {Moment Tensor Potentials: A Class of Systematically Improvable Interatomic Potentials},
journal = {Multiscale Modeling \& Simulation},
volume = {14},
number = {3},
pages = {1153-1173},
year = {2016},
doi = {10.1137/15M1054183},

}

@article{CHAPMAN2020109483,
title = {Machine learning models for the prediction of energy, forces, and stresses for Platinum},
journal = {Computational Materials Science},
volume = {174},
pages = {109483},
year = {2020},
issn = {0927-0256},
author = {J. Chapman and R. Batra and R. Ramprasad},
}

@Article{Park2021,
author={Park, Cheol Woo
and Kornbluth, Mordechai
and Vandermause, Jonathan
and Wolverton, Chris
and Kozinsky, Boris
and Mailoa, Jonathan P.},
title={Accurate and scalable graph neural network force field and molecular dynamics with direct force architecture},
journal={npj Computational Materials},
year={2021},
month={May},
day={21},
volume={7},
number={1},
pages={73},
}

@Article{Chan2020,
author={Chan, Henry
and Cherukara, Mathew
and Loeffler, Troy D.
and Narayanan, Badri
and Sankaranarayanan, Subramanian K. R. S.},
title={Machine learning enabled autonomous microstructural characterization in 3D samples},
journal={npj Computational Materials},
year={2020},
month={Jan},
day={06},
volume={6},
number={1},
pages={1},
}

@article{GUPTA202110927,
title = {Graph neural network: Current state of Art, challenges and applications},
journal = {Materials Today: Proceedings},
volume = {46},
pages = {10927-10932},
year = {2021},
note = {International Conference on Technological Advancements in Materials Science and Manufacturing},
issn = {2214-7853},

author = {Atika Gupta and Priya Matta and Bhasker Pant},

}


@article{Steinbach_2009,
	doi = {10.1088/0965-0393/17/7/073001},
	url = {https://doi.org/10.1088/0965-0393/17/7/073001},
	year = 2009,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {17},
	number = {7},
	pages = {073001},
	author = {Ingo Steinbach},
	title = {Phase-field models in materials science},
	journal = {Modelling and Simulation in Materials Science and Engineering},

}

@article{https://doi.org/10.1002/ar.a.20169,
author = {Richmond, Brian G. and Wright, Barth W. and Grosse, Ian and Dechow, Paul C. and Ross, Callum F. and Spencer, Mark A. and Strait, David S.},
title = {Finite element analysis in functional morphology},
journal = {The Anatomical Record Part A: Discoveries in Molecular, Cellular, and Evolutionary Biology},
volume = {283A},
number = {2},
pages = {259-274},
keywords = {finite-element analysis, mastication, primates, biomechanics, functional morphology, paleoanthropology},
doi = {https://doi.org/10.1002/ar.a.20169},
year = {2005}
}

@article{KAVOUSI2022126461,
title = {A temperature-dependent atomistic-informed phase-field model to study dendritic growth},
journal = {Journal of Crystal Growth},
volume = {579},
pages = {126461},
year = {2022},
issn = {0022-0248},
doi = {https://doi.org/10.1016/j.jcrysgro.2021.126461},
}


@article{doi:10.1080/00018730701822522,
author = { Heike   Emmerich },
title = {Advances of and by phase-field modelling in condensed-matter physics},
journal = {Advances in Physics},
volume = {57},
number = {1},
pages = {1-87},
year  = {2008},
publisher = {Taylor & Francis},
doi = {10.1080/00018730701822522},

URL = { 
        https://doi.org/10.1080/00018730701822522
    
},
eprint = { 
        https://doi.org/10.1080/00018730701822522
    
}

}


@Article{Farrahi2020,
author={Farrahi, Gholam Hossein
and Javanbakht, Mahdi
and Jafarzadeh, Hossein},
title={On the phase field modeling of crack growth and analytical treatment on the parameters},
journal={Continuum Mechanics and Thermodynamics},
year={2020},
month={May},
day={01},
volume={32},
number={3},
pages={589-606},
issn={1432-0959},
doi={10.1007/s00161-018-0685-z},

}

@article{PLIMPTON19951,
title = {Fast Parallel Algorithms for Short-Range Molecular Dynamics},
journal = {Journal of Computational Physics},
volume = {117},
number = {1},
pages = {1-19},
year = {1995},
issn = {0021-9991},
doi = {https://doi.org/10.1006/jcph.1995.1039},
url = {https://www.sciencedirect.com/science/article/pii/S002199918571039X},
author = {Steve Plimpton}
}


@article{ZHOU20014005,
title = {Atomic scale structure of sputtered metal multilayers},
journal = {Acta Materialia},
volume = {49},
number = {19},
pages = {4005-4015},
year = {2001},
issn = {1359-6454},
doi = {https://doi.org/10.1016/S1359-6454(01)00287-7},
author = {X.W. Zhou and H.N.G. Wadley and R.A. Johnson and D.J. Larson and N. Tabat and A. Cerezo and A.K. Petford-Long and G.D.W. Smith and P.H. Clifton and R.L. Martens and T.F. Kelly},

}

@article{ase-paper,
  author={Ask Hjorth Larsen and Jens Jørgen Mortensen and Jakob Blomqvist and Ivano E Castelli and Rune Christensen and Marcin
Dułak and Jesper Friis and Michael N Groves and Bjørk Hammer and Cory Hargus and Eric D Hermes and Paul C Jennings and Peter
Bjerre Jensen and James Kermode and John R Kitchin and Esben Leonhard Kolsbjerg and Joseph Kubal and Kristen
Kaasbjerg and Steen Lysgaard and Jón Bergmann Maronsson and Tristan Maxson and Thomas Olsen and Lars Pastewka and Andrew
Peterson and Carsten Rostgaard and Jakob Schiøtz and Ole Schütt and Mikkel Strange and Kristian S Thygesen and Tejs
Vegge and Lasse Vilhelmsen and Michael Walter and Zhenhua Zeng and Karsten W Jacobsen},
  title={The atomic simulation environment—a Python library for working with atoms},
  journal={Journal of Physics: Condensed Matter},
  volume={29},
  number={27},
  pages={273002},
  url={http://stacks.iop.org/0953-8984/29/i=27/a=273002},
  year={2017},

}

@incollection{NEURIPS2019_9015,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
}


@article{ELFWING20183,
title = {Sigmoid-weighted linear units for neural network function approximation in reinforcement learning},
journal = {Neural Networks},
volume = {107},
pages = {3-11},
year = {2018},
note = {Special issue on deep reinforcement learning},
issn = {0893-6080},
doi = {https://doi.org/10.1016/j.neunet.2017.12.012},
author = {Stefan Elfwing and Eiji Uchibe and Kenji Doya},

}


@inproceedings{NEURIPS2019_2f4fe03d,
 author = {Xu, Jingjing and Sun, Xu and Zhang, Zhiyuan and Zhao, Guangxiang and Lin, Junyang},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Understanding and Improving Layer Normalization},
 url = {https://proceedings.neurips.cc/paper/2019/file/2f4fe03d77724a7217006e5d16728874-Paper.pdf},
 volume = {32},
 year = {2019}
}


@article{HIREL2015212,
title = {Atomsk: A tool for manipulating and converting atomic data files},
journal = {Computer Physics Communications},
volume = {197},
pages = {212-219},
year = {2015},
issn = {0010-4655},
doi = {https://doi.org/10.1016/j.cpc.2015.07.012},
author = {Pierre Hirel},

}

@Article{chapman2021sgop,
author={Chapman, James
and Goldman, Nir
and Wood, Brandon C.},
title={Efficient and universal characterization of atomic structures through a topological graph order parameter},
journal={npj Computational Materials},
year={2022},
month={Mar},
day={11},
volume={8},
number={1},
pages={37},
issn={2057-3960},
doi={10.1038/s41524-022-00717-7},
url={https://doi.org/10.1038/s41524-022-00717-7}
}


@article{pozdnyakov_local_2021,
	title = {Local invertibility and sensitivity of atomic structure-feature mappings},
	journal = {Preprint at http://arxiv.org/abs/2109.11440},
	author = {Pozdnyakov, Sergey N. and Zhang, Liwei and Ortner, Christoph and Csányi, Gábor and Ceriotti, Michele},
	year = {2021},
}


@article{sullivan2019pyvista,
  doi = {10.21105/joss.01450},
  url = {https://doi.org/10.21105/joss.01450},
  year = {2019},
  month = {May},
  publisher = {The Open Journal},
  volume = {4},
  number = {37},
  pages = {1450},
  author = {C. Bane Sullivan and Alexander Kaszynski},
  title = {{PyVista}: {3D} plotting and mesh analysis through a streamlined interface for the {Visualization Toolkit} ({VTK})},
  journal = {Journal of Open Source Software}
}


@article{klicpera2020directional,
  title={Directional message passing for molecular graphs},
  author={Klicpera, Johannes and Gross, Janek and Gunnemann, Stephan},
  journal={arXiv preprint arXiv:2003.03123},
  year={2020}
}

@article{https://doi.org/10.1002/anie.201902625,
author = {Bernstein, Noam and Bhattarai, Bishal and Csányi, Gábor and Drabold, David A. and Elliott, Stephen R. and Deringer, Volker L.},
title = {Quantifying Chemical Structure and Machine-Learned Atomic Energies in Amorphous and Liquid Silicon},
journal = {Angewandte Chemie International Edition},
volume = {58},
number = {21},
pages = {7057-7061},
keywords = {amorphous materials, computational chemistry, continuous random networks, machine learning, silicon},
year = {2019}
}

@article{GUO2016624,
title = {Fe-based amorphous coating for corrosion protection of magnesium alloy},
journal = {Materials and Design},
volume = {108},
pages = {624-631},
year = {2016},
author = {S.F. Guo and F.S. Pan and H.J. Zhang and D.F. Zhang and J.F. Wang and J. Miao and C. Su and C. Zhang},


}


@article{
doi:10.1126/science.1078616,
author = {Y. Lin  and H. Skaff  and T. Emrick  and A. D. Dinsmore  and T. P. Russell },
title = {Nanoparticle Assembly and Transport at Liquid-Liquid Interfaces},
journal = {Science},
volume = {299},
number = {5604},
pages = {226-229},
year = {2003},

}

@article{https://doi.org/10.1002/adma.200800440,
author = {Wacaser, Brent A. and Dick, Kimberly A. and Johansson, Jonas and Borgström, Magnus T. and Deppert, Knut and Samuelson, Lars},
title = {Preferential Interface Nucleation: An Expansion of the VLS Growth Mechanism for Nanowires},
journal = {Advanced Materials},
volume = {21},
number = {2},
pages = {153-165},
year = {2009}
}

@article{doi:10.1021/la052551e,
author = {Willner, Itamar and Katz, Eugenii},
title = {Controlling Chemical Reactivity at Solid-Solution Interfaces by Means of Hydrophobic Magnetic Nanoparticles},
journal = {Langmuir},
volume = {22},
number = {4},
pages = {1409-1419},
year = {2006},


}

@article{GITTLEMAN201981,
title = {Materials research and development focus areas for low cost automotive proton-exchange membrane fuel cells},
journal = {Current Opinion in Electrochemistry},
volume = {18},
pages = {81-89},
year = {2019},
note = {Energy Storage Energy Transformation},
author = {Craig S. Gittleman and Anusorn Kongkanand and David Masten and Wenbin Gu},

}

@article{https://doi.org/10.1002/adma.201805876,
author = {Abbasi, Reza and Setzler, Brian P. and Lin, Saisai and Wang, Junhua and Zhao, Yun and Xu, Hui and Pivovar, Bryan and Tian, Boyuan and Chen, Xi and Wu, Gang and Yan, Yushan},
title = {A Roadmap to Low-Cost Hydrogen with Hydroxide Exchange Membrane Electrolyzers},
journal = {Advanced Materials},
volume = {31},
number = {31},
pages = {1805876},
year = {2019}
}

@Article{Mahmood2022,
author={Mahmood, Yasir
and Alghalayini, Maher
and Martinez, Enrique
and Paredis, Christiaan J. J.
and Abdeljawad, Fadi},
title={Atomistic and machine learning studies of solute segregation in metastable grain boundaries},
journal={Scientific Reports},
year={2022},
month={Apr},
day={23},
volume={12},
number={1},
pages={6673},
doi={10.1038/s41598-022-10566-5},
}

@article{heo2021microstructural,
  title={Microstructural impacts on ionic conductivity of oxide solid electrolytes from a combined atomistic-mesoscale approach},
  author={Heo, Tae Wook and Grieder, Andrew and Wang, Bo and Wood, Marissa and Hsu, Tim and Akhade, Sneha A and Wan, Liwen F and Chen, Long-Qing and Adelstein, Nicole and Wood, Brandon C},
  journal={npj Computational Materials},
  volume={7},
  number={1},
  pages={1--15},
  year={2021},
  publisher={Nature Publishing Group}
}

@Article{Heo2021,
author={Heo, Tae Wook
and Grieder, Andrew
and Wang, Bo
and Wood, Marissa
and Hsu, Tim
and Akhade, Sneha A.
and Wan, Liwen F.
and Chen, Long-Qing
and Adelstein, Nicole
and Wood, Brandon C.},
title={Microstructural impacts on ionic conductivity of oxide solid electrolytes from a combined atomistic-mesoscale approach},
journal={npj Computational Materials},
year={2021},
month={Dec},
day={21},
volume={7},
number={1},
pages={214},
issn={2057-3960},
doi={10.1038/s41524-021-00681-8},
}

@article{HEO201468,
title = {Phase-field modeling of displacive phase transformations in elastically anisotropic and inhomogeneous polycrystals},
journal = {Acta Materialia},
volume = {76},
pages = {68-81},
year = {2014},
issn = {1359-6454},
doi = {https://doi.org/10.1016/j.actamat.2014.05.014},
url = {https://www.sciencedirect.com/science/article/pii/S1359645414003620},
author = {Tae Wook Heo and Long-Qing Chen},
keywords = {Displacive phase transformation, Inhomogeneous elasticity, Elastic anisotropy, Polycrystals, Phase-field model},
}

@article{HEO2019262,
title = {A phase-field model for hydride formation in polycrystalline metals: Application to $\gamma$-hydride in zirconium alloys},
journal = {Acta Materialia},
volume = {181},
pages = {262-277},
year = {2019},
issn = {1359-6454},
doi = {https://doi.org/10.1016/j.actamat.2019.09.047},
url = {https://www.sciencedirect.com/science/article/pii/S1359645419306378},
author = {Tae Wook Heo and Kimberly B. Colas and Arthur T. Motta and Long-Qing Chen},
keywords = {Metal–hydrogen interactions, Hydride formation, Polycrystals, Zirconium hydrides, Phase-field model},
}







@article{doi:10.1146/annurev.matsci.32.112001.132041,
author = {Chen, Long-Qing},
title = {Phase-Field Models for Microstructure Evolution},
journal = {Annual Review of Materials Research},
volume = {32},
number = {1},
pages = {113-140},
year = {2002},
doi = {10.1146/annurev.matsci.32.112001.132041},

}

@article{doi:10.1146/annurev.matsci.32.101901.155803,
author = {Boettinger, W. J. and Warren, J. A. and Beckermann, C. and Karma, A.},
title = {Phase-Field Simulation of Solidification},
journal = {Annual Review of Materials Research},
volume = {32},
number = {1},
pages = {163-194},
year = {2002},
doi = {10.1146/annurev.matsci.32.101901.155803},

}

@article{Heo_2021,
	doi = {10.1088/2515-7639/abeef8},
	url = {https://doi.org/10.1088/2515-7639/abeef8},
	year = 2021,
	month = {jun},
	publisher = {{IOP} Publishing},
	volume = {4},
	number = {3},
	pages = {034012},
	author = {Tae Wook Heo and Saad A Khairallah and Rongpei Shi and Joel Berry and Aurelien Perron and Nicholas P Calta and Aiden A Martin and Nathan R Barton and John Roehling and Tien Roehling and Jean-Luc Fattebert and Andy Anderson and Albert L Nichols and Steven Wopschall and Wayne E King and Joseph T McKeown and Manyalibo J Matthews},
	title = {A mesoscopic digital twin that bridges length and time scales for control of additively manufactured metal microstructures},
	journal = {Journal of Physics: Materials},
}












